Combining Machine Learning and Computational Chemistry for Predictive Insights Into Chemical Systems

Machine learning models are poised to make a transformative impact on chemical sciences by dramatically accelerating computational algorithms and amplifying insights available from computational chemistry methods. However, achieving this requires a confluence and coaction of expertise in computer science and physical sciences. This review is written for new and experienced researchers working at the intersection of both fields. We first provide concise tutorials of computational chemistry and machine learning methods, showing how insights involving both can be achieved. We then follow with a critical review of noteworthy applications that demonstrate how computational chemistry and machine learning can be used together to provide insightful (and useful) predictions in molecular and materials modeling, retrosyntheses, catalysis, and drug design.

==> ChemRevNotes.tex <==

-- should be substantial, comprehensive, authoritative, critical, and readable
-- items that have not been comprehensively and critically reviewed in the past three to four years
-- Reviews of general interest and with high potential for broad impact are preferable to narrowly focused ones.
-- Scope and time period must be clearly defined in the introduction.
-- the author’s own work should not be singled out for emphasis
-- addressed to readers who are competent in fundamentals but need not have extensive knowledge of the topic
-- comprehensive, but no specific style or length 
-- must give analysis and insights about remaining challenges and future directions

----

The Focus Review is a special type of manuscript that is distinct from a regular review because it is more concise and forward looking and typically addresses a rapidly evolving topic. These types of reviews must still retain the key characteristics associated with Chemical Reviews. Specifically, a Focus Review must be comprehensive within the scope defined in the Introduction, even if this scope is relatively narrow, and should not single out the author’s own work for emphasis but rather should consider all significant contributions to the field. It must also contain a critical analysis, as well as a discussion of remaining challenges and future directions. A Focus Review should be no longer than 20 published pages, which corresponds to approximately 60 double-spaced submitted manuscript pages, including embedded figures, tables, and references. As with regular Reviews, a Focus Review can be submitted either on the invitation of an Editor, or after submitting a proposal and receiving approval from the editors as described above. The criteria for publishing a Focus Review will be especially rigorous to maintain a high level of quality. Moreover, a Focus Review must be concise, and if a submitted Focus Review becomes too long, it may be converted to a regular review by the Editor handling the manuscript.

----

The Introduction, usually one or two manuscript pages, should state precisely the purpose and goals of the review and its scope and limitations, as well as the years of literature covered. Historical material and references to earlier pertinent reviews may be included. Any special nomenclature, notation, or symbols should be defined here.


==> Sections/GlossaryList.tex <==
\begin{enumerate}
    \item Representation -- 
    \item Clever Hans -- 
    \item Full Configuration Interaction -- 
    \item Multireference wavefunction method -- 
\end{enumerate}

==> Sections/ML_heatmap_keywords.tex <==
#ACS Divisions
#Agricultural & Food Chemistry (AGFD)
#Agrochemicals (AGRO)
#Analytical Chemistry (ANYL)
#Biochemical Technology (BIOT)
#Biological Chemistry (BIOL)
#Business Development & Management (BMGT)
#Carbohydrate Chemistry (CARB)
#Catalysis Science and Technology (CATL)
#Cellulose and Renewable Materials (CELL)
#Chemical Education (CHED)
#Chemical Health & Safety (CHAS)
#Chemical Information (CINF)
#Chemical Toxicology (TOXI)
#Chemistry & the Law (CHAL)
#Colloid & Surface Chemistry (COLL)
#Computers in Chemistry (COMP)
#Energy & Fuels (ENFL)
#Environmental Chemistry (ENVR)
#Fluorine Chemistry (FLUO)
#Geochemistry (GEOC)
#History of Chemistry (HIST)
#Industrial & Engineering Chemistry (I&EC)
#Inorganic Chemistry (DIC) or (INOR)
#Medicinal Chemistry (MEDI)
#Nuclear Chemistry & Technology (NUCL)
#Organic Chemistry (ORGN)
#Physical Chemistry (PHYS)
#Polymer Chemistry (POLY)
#Polymeric Materials: Science & Engineering (PMSE)
#Professional Relations (PROF)
#Rubber (RUBB)
#Small Chemical Businesses (SCHB)
divisions = {'AGFD': {'name': 'agricultural and food chemistry',
  'keywords': ['agricultur*',
   'food',
   'microbiological hazard*',
   'metabolomic*',
   'antibiotic*',
   'breath monitoring',
   'chocolate*',
   'traditional chinese medicine',
   'wine',
   'nut*',
   'allergen*',
   'fresh produce',
   'cereal*',
   'gut microbiome*',
   'biomass',
   'biosensor*',
   'sensory evaluation',
   'endocrine disrupting',
   'ferment*',
   'nanoencapsulation',
   'bioactive',
   'pectin*',
   'beer',
   'spirits',
   'edible',
   'phenolic*',
   'phytochemical*',
   'biopolymer*',
   'nutrition*',
   'microbiome',
   'dietary',
   'fungicide*',
   'huanglongbing',
   'flavor',
   'space travel',
   'extreme environment*',
   'fruit*',
   'tea',
   'cotton',
   'seafood*',
   'nutrient*',
   'artisanal',
   'vegetable*',
   'coffee',
   'cocoa',
   'protein*']},
 'AGRO': {'name': 'agrochemicals',
  'keywords': ['agrochemical',
   'agrochemicals',
   'cannabis',
   'insecticide*',
   'hemp',
   'developing countr*',
   'glyphosate',
   'degradant*',
   'agroecosystem*',
   'pesticide*',
   'soil',
   'microplastic*',
   'stereoisomer*',
   'fumigant*',
   'crop*',
   'pollinator',
   'semiochemical',
   'metabolite*',
   'surface water',
   'groundwater',
   'water sediment interface',
   'habitat protection',
   'herbicide*',
   'neonicotinoid*',
   'xenobiotic*',
   'agricultural emission*',
   'ecotoxicity',
   'veterinary drug*']},
 'ANYL': {'name': 'analytical chemistry',
  'keywords': ['analytical chemistry',
   'spectrometry',
   'analytical separation*',
   'sensor*',
   'nanotechnology',
   'nanozyme*',
   'spectroscopy',
   'biosensing',
   'chemical forensic*',
   'chemometric*',
   'groundwater',
   'chemical identification',
   'bioanaly*',
   'chemical assay*',
   'characterization*',
   'organic analys*',
   'biosensor*',
   'proteomic*',
   'chromatography',
   'blood based diagnostic*',
   'cancer detection']},
 'BIOT': {'name': 'biochemical technology',
  'keywords': ['biochemi*',
   'biotechnology',
   'bioengineering',
   'biomedical technolog*',
   'chemical biology',
   'chromatographic separation*',
   'drug delivery',
   'biotherapeutic*',
   'precision medicine',
   'protein engineering',
   'bioprocess*',
   'systems biology',
   'synthetic biology',
   'biomanufacturing',
   'biophysic*',
   'bio based product*',
   'biological chem*']},
 'BIOL': {'name': 'biological chemistry',
  'keywords': ['biological chemistry',
   'cytochrome*',
   'biomolecule*',
   'bioorthogonal chem*',
   'enzyme chem*',
   'RNA based therap*',
   'bioconjugate',
   'drug discovery',
   'structural biology',
   'chemical signaling',
   'protein folding',
   'protein aggregation',
   'organofluorine',
   'genome engineering',
   'biosynthesis',
   'chem* biology']},
 'BMGT': {'name': 'business development and management',
  'keywords': ['chem* business*',
   'chem* compan*',
   'chem* enterprise*',
   'chem* research and development']},
 'CARB': {'name': 'carbohydrate chemistry',
  'keywords': ['carbohydrate*',
   'oligosaccharide*',
   'glycoconjugate*',
   'glycobiology',
   'glycan*',
   'glycoscience*',
   'protein o-glcnacylation',
   'glycoprotein*',
   'nucleic acid* based therap*',
   'glycomimetics']},
 'CATL': {'name': 'catalysis science and technology',
  'keywords': ['cataly*',
   'electrocataly*',
   'photocataly*',
   'scaling relation*',
   'surface science',
   'surface kinetic*',
   'surface mechanism*',
   'surface reaction*',
   'metal support*',
   'amorphous material*',
   'nanoporous material*',
   'syngas conversion',
   'metal oxides',
   'disordered material*',
   'methane conversion',
   'mixed metal oxide*',
   'vehicle emission control',
   'surface chemistry',
   'material* genome']},
 'CELL': {'name': 'cellulose and renewable materials',
  'keywords': ['cellulose',
   'nanocellulose*',
   'renewable material*',
   'polysaccharide*',
   'colloidal assembl*',
   'lignin',
   'lignocellulos*',
   'hemp']},
 'CHED': {'name': 'chemical education',
  'keywords': ['chem* educat*',
   'data literacy',
   'chem* curricul*',
   'chem* student*',
   'chem* educat*',
   'learn* in the laboratory',
   'climate change literacy',
   'lab* safety',
   'chem* class*',
   'chem* communication*']},
 'CHAS': {'name': 'chemical health and safety',
  'keywords': ['chem* safety',
   'lab* safety',
   'chem* regulations',
   'environmental health and safety']},
 'CINF': {'name': 'chemical information',
  'keywords': ['chemical informatics',
   'bio* modeling',
   'computational chemistry',
   'cheminformatic*',
   'chemical info*',
   'drug discovery',
   'chem* database*',
   'chem* librar*',
   'chem* vocabulary',
   'materials informatic*']},
 'TOXI': {'name': 'chemical toxicology',
  'keywords': ['toxi*', 'antibody drug conjugate*', 'chemical exposure*']},
 'CHAL': {'name': 'chemistry and the law',
  'keywords': ['chem* patent*',
   'pharmaceutical patent*',
   'chem* in commerce']},
 'COLL': {'name': 'colloid and surface chemistry',
  'keywords': ['colloid*',
   'surface chemistry',
   'surface science',
   'surfactant*',
   'biomaterial*',
   'biointerface*',
   'nanomaterial*',
   'coating material*',
   'biomembrane*',
   'nanoparticle*',
   'polymer system*',
   'adsorption',
   'surface reaction*',
   'tribolog*',
   'nanomedicine*',
   'low dimensional material*',
   'molecular electronic*',
   'mechanochem*',
   'tribochem*',
   'emuls*',
   'nanotheranostic*',
   'coacerv*',
   'nanostructure',
   'monolayer*',
   'bilayer*',
   'thin film*']},
 'COMP': {'name': 'computers in chemistry',
  'keywords': ['chem* comput*',
   'drug design',
   'drug discovery',
   'computational chem*',
   'molecular mechanics',
   'multiscale modeling',
   'computational quantum chem*',
   'quantum comp*',
   'quantum dynamic*',
   'multiscale computational modeling',
   'computational model* of chem*',
   'chem* database*',
   'material* database*',
   'protein database*',
   'rna design*',
   'density functional theory',
   'computational cataly*',
   'molecular model*',
   'chem* librar*',
   'chem* screen*',
   'molecular recognition',
   'computer-aided peptide design']},
 'ENFL': {'name': 'energy and fuels',
  'keywords': ['energy and fuel*',
   'energy application*',
   'fuel*',
   'hydrocracking',
   'hydrotreating',
   'waste feedstock*',
   'energy technolog*',
   '*material* for energy',
   'gas separation*',
   'gas storage',
   'gas utilization',
   'hybrid solar cell*',
   'fuel* design',
   'aviation fuel*',
   'hydraulic frac*',
   'batter*',
   'bioenergy',
   'petroleum',
   'methane',
   'natural gas*',
   'lithium ion',
   'resource recovery',
   'energy conversion*',
   'hybrid energy',
   'porous material*',
   'environment* sustain*',
   'photocataly*',
   'biofuel*',
   'bio based product*',
   'energy material*',
   'carbon dioxide conversion',
   'carbon dioxide utilization',
   'renewable energy',
   'energy storage',
   'electrochemical',
   'solar energy',
   'artificial photosynthesis',
   'resource production',
   'oil industry',
   'gas industry',
   'oil and gas industry',
   'fuel cell*',
   'hybrid vehicle*',
   'cataly*',
   'solar cell',
   'water splitting',
   'hydrogen generation',
   'gas hydrate*',
   'shale gas',
   'energy efficiency',
   'bio based chemical*',
   'hydrogen energy',
   'carbon management',
   'geothermal energy']},
 'ENVR': {'name': 'environmental chemistry',
  'keywords': ['environmental chem*',
   'atmospher* chem*',
   'biomimetic membrane*',
   'cataly*',
   'water treatment',
   'water purification',
   'plastic* recycling',
   'emerging contaminant*',
   'disinfection byproduct*',
   'environmental health',
   'two dimensional nanomaterial*',
   'environmental implication*',
   'water quality',
   'water distribution',
   'water infrastructure',
   'water pollution',
   'agricultural waste*',
   'environmental monitor*',
   'environmental remediation*',
   'nanomaterial* in the environment',
   'environmental science',
   'biogeochemical transformation',
   'water contaminant*',
   'environment* research',
   'green chem*',
   'environmental bioprocess*',
   'micro plastic*',
   'stormwater',
   'environmental sustainability',
   'water channel*',
   'water purification',
   'water desalination',
   'biochar',
   'hydrochar',
   'water sustainability',
   'water analysis',
   'wastewater',
   'dissolved organic matter',
   '*sensor*',
   'green infrastructure',
   'soil*',
   'nanotechnology',
   'photooxidation',
   'water source*',
   'fertilizer*',
   'drinking water',
   'organic contaminant*',
   'microplastic pollution',
   'nanobubble*',
   'separation of salt*',
   'radionuclide*',
   'trace organic contaminant*',
   'soil plant system*',
   'nanotoxicology',
   'clay mineral*',
   'pesticides in surface water']},
 'FLUO': {'name': 'fluorine chemistry',
  'keywords': ['fluorine*', 'radiopharmaceutical chem*']},
 'GEOC': {'name': 'geochemistry',
  'keywords': ['*geochem*',
   'iron oxide*',
   'inorganic solid*',
   'oil and gas development',
   'manganese oxide*',
   'contaminated soil',
   'groundwater',
   'geogenic',
   'anthropogenic',
   'clathrate hydrate',
   'geological process*',
   'mineral dissolution',
   'contaminated site remediation',
   'biomineralization',
   'hydraulic frac*',
   'soil ecosystem*',
   'unconventional oil and gas development',
   'cementitious material*']},
 'HIST': {'name': 'history of chemistry',
  'keywords': ['chem* histor*', 'history of chem*', 'evolution of chem*']},
 'I&EC': {'name': 'industrial and engineering chemistry',
  'keywords': ['industrial and engineering chemistry',
   'industrial chem*',
   'molten salt*',
   'recycling material*',
   'material* recovery',
   'water desalination',
   'rare earth element*',
   'chem* industrial application*',
   'separation science*',
   'water purification',
   'industrial and engineering chemistry']},
 'INOR': {'name': 'inorganic chemistry',
  'keywords': ['*inorganic chem*',
   'organometallic*',
   'phosphorus chem*',
   'metallodrug*',
   '*inorganic cataly*',
   'chemistry of material*',
   'metal organic framework*',
   'nanomaterial*',
   'coordination chem*',
   'electrochem*',
   'lanthanide*',
   'actinide*',
   'electrocataly*',
   'nanoscience*',
   'metal nanostructure*',
   'solid state phenomen*']},
 'MEDI': {'name': 'medicinal chemistry',
  'keywords': ['medic* chem*',
   'drug discovery',
   'immunomodulator*',
   'lipophil*',
   'protein degradation',
   'sulfonamide*',
   'glioblastoma*',
   'pancreatic cancer',
   'drug design',
   'protein interaction*',
   'neurodegeneration',
   'targeting rna',
   'brain penetration',
   'neuro-oncology',
   'opioid epidemic',
   'gasotransmitter*',
   'pi3k inhibitor*',
   'atropisomer*',
   'cyp450 enzyme*',
   'muscarinic receptor*',
   'hiv 1 infection',
   'neuropathic pain',
   'antibiotic*',
   'kinase inhibitor*',
   'macrocycle*',
   'cyclopeptide*',
   'misfolded protein*']},
 'NUCL': {'name': 'nuclear chemistry and technology',
  'keywords': ['nuclear tech*',
   'nuclear chem*',
   'actinide*',
   'radiochem*',
   'nuclear waste',
   'nuclear forensic*',
   'radioisotope*',
   'nuclear fuel*',
   'lanthanide*',
   'radiotherapeutic*',
   'nuclear reaction*',
   'molten salt reactor*',
   'concentrated electrolyte*',
   'nuclear medicine*',
   'isotope*',
   'accelerator facilit*',
   'curium',
   'nuclear fission']},
 'ORGN': {'name': 'organic chemistry',
  'keywords': ['organic chem*',
   'organic synthes*',
   'asymmetric reaction*',
   'asymmetric synthes*',
   'biocataly*',
   'carbon allotrope*',
   'cross coupling reaction*',
   'heterocycle*',
   'aromatic*',
   'organic electrochem*',
   'molecular recognition',
   'molecular self assembly',
   'organometallic*',
   'peptide*',
   'protein*',
   'amino acid*',
   'photoredox',
   'complex molecule*',
   'enzyme engineering',
   'synthetic chem*',
   'organic molecule*',
   'polymer chem*',
   'carbon nanotube* chem*',
   'graphene chem*',
   'organic electronic*',
   'amide bond*',
   'chemical biology']},
 'PHYS': {'name': 'physical chemistry',
  'keywords': ['physical chem*',
   'nonlinear optic*',
   'electrochem*',
   'biomolecular structure*',
   'biomolecular dynamic*',
   'biophysic*',
   'ion*',
   '2d material*',
   'two dimensional material*',
   'amyloid',
   'graph theory',
   'molecular electronic*',
   'optical imaging',
   'electro*',
   'materials for energy',
   'molecular assembl*',
   'biomaterial*',
   'biomolecular structure*',
   'microscopy',
   'spectroscopy',
   'redox flow batter*',
   'computational molecular science',
   'exciton*',
   'astrochem*',
   'density functional theory',
   'chiral*',
   'nano*',
   'enzyme specificity',
   'enzyme promiscuity',
   'liquid theory',
   'membrane protein*',
   'molecular fluid*',
   'photoactivit*',
   'atom*',
   'quantum*']},
 'POLY': {'name': 'polymer chemistry',
  'keywords': ['polymer*',
   'polyolefin*',
   'biomacromolecule*',
   'macromolecule*',
   'plastic*',
   'polymeriz*',
   'polymeric',
   'block copolymer*',
   'poly 2 oxazoline*',
   'biomimicry',
   'lignin']},
 'PMSE': {'name': 'polymeric materials: science and engineering',
  'keywords': ['polymer* material*',
   'polymer* science',
   '*polymer*',
   'coating material*',
   'thin film*',
   'polyolefin*',
   'macromolecul*',
   'tissue engineering',
   '*peptide*',
   'nanoclay*',
   'polyelectrolyte*',
   'polyphosphazene*']},
 'PROF': {'name': 'professional relations', 'keywords': ['chem* education']},
 'RUBB': {'name': 'rubber', 'keywords': ['rubber*']},
 'SCHB': {'name': 'small chemical businesses',
  'keywords': ['chem* sector*',
   'academic entrepreneur*',
   'commercial chem*',
   'science advoca*']}}
   

==> Sections/desc_table.tex <==
\pagebreak
\begin{tiny}
\begin{longtable}{llcclcc}
\label{tab:descriptors}
\caption{Atomistic systems can be represented in a myriad of ways. Some descriptions are designed to emphasise particular aspects of a system, while others aim to disambiguate similar chemical or physical principles across a wide range of molecules or materials. The set of desirable properties in a representation thus depends on the task at hand. The following overview gives a coarse characterization of the most popular representations.
We distinguish between four computational efficiency classes $\circled{A} - \circled{D}$ in descending order, depending on the number of considered many-body terms in the descriptor. The efficiency class additionally reflects if a representation relies on particularly expensive operations (e.g. a hierarchical processing or matching of inputs).
Furthermore, we indicate if a representation is unique and able to encode any physical state of the system unambiguously. Note, that this property may not be crucial in practice, because ML models only have to generalize across a relatively narrow scope of inputs.
The symbols \CheckmarkBold{} and \ding{56} show if a descriptor satisfies a certain property or not, while \Circle{} means that a property is partly satisfied.}\\

& \toprule
\endfirsthead
% if contintues is not desired comment out the following 3 lines and change \endfirsthead to \endhead
\caption[]{(continued)}\\
\toprule
\endhead

\textbf{Descriptors} & \textbf{Comp. efficiency} & \textbf{Periodic}  & \textbf{Uniq.}  & \textbf{Invariances} & \textbf{Global} & \textbf{Smooth}\\
\toprule
%\multicolumn{7}{l}{} \\
%\multicolumn{7}{l}{} \\
%\toprule
\multirow{3}{3cm}{Atom-centered Symmetry Functions (ASCF)~\cite{behler2011atom}}  & \multirow{3}{*}{\circled{B} 1,2,3-body terms, cut-off} & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Smooth Overlap of Atomic Positions (SOAP)~\cite{0444_Bartok2013}} & \multirow{3}{3cm}{\circled{B} density based, $\text{SO}_3$ integration} & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}   & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Coulomb Matrix (CM)~\cite{rupp2012fast}} & \multirow{3}{*}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\CheckmarkBold{}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \ding{56} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Sine Matrix~\cite{faber2015crystal}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \ding{56} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Ewald Sum Matrix~\cite{faber2015crystal}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \ding{56} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Bag of Bonds (BoB)~\cite{0161_Hansen2015}}  & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\ding{56}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \Circle{} permutations\footnote{Partial permutation invariance via feature sorting}  &  & \\
\midrule
\multirow{3}{3cm}{Faber-Christensen-Huang-Lilienfeld (FCHL)~\cite{christensen2020fchl}} & \multirow{3}{3cm}{\circled{C} 1,2,3-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule 
\multirow{3}{3cm}{Spectrum of London and Axilrod-Teller-Muto potential (SLATM)~\cite{faber2018alchemical}} & \multirow{3}{3cm}{\circled{D} 1,2,3,4-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
   &  &  &  & \CheckmarkBold{} rotations  &  & \\
   &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Many-body Tensor Representation (MBTR)~\cite{huo2017unified}} & \multirow{3}{3cm}{\circled{C} 1,2,3-body terms} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} &
\CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Atomic cluster expansion~\cite{drautz2019atomic}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\bottomrule

\pagebreak

\textbf{NN architectures} & \textbf{Comp. efficiency} & \textbf{Periodic}  & \textbf{Uniq.}  & \textbf{Invariances} & \textbf{Global} & \textbf{Smooth}\\
\toprule
%\multicolumn{7}{l}{} \\
%\multicolumn{7}{l}{\textbf{NN architectures}} \\
%\toprule
\multirow{3}{3cm}{Deep Potential - Smooth Edition (DeepPot-SE)~\cite{zhang2018deep,zhang2018end}} & \multirow{3}{3cm}{\circled{B} 1,2,3-body terms, cut-off} & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{MPNN/SchNet~\cite{0336_schutt2017quantum,0338_schutt2018schnet}} & \multirow{3}{3cm}{\circled{B} 1,2-body terms, hierarchical} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Cormorant~\cite{anderson2019cormorant}} & \multirow{3}{3cm}{\circled{B} 1,2-body terms, hierarchical} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  &  \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Tensor Field Networks~\cite{thomas2018tensor}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\bottomrule

\multicolumn{7}{l}{} \\
\multicolumn{7}{l}{\textbf{Similarity metrics}} \\
\toprule

\multirow{3}{3cm}{Root mean square deviation of atomic positions (RMSD)~\cite{sadeghi2013metrics}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\ding{56}} 
& \Circle{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
  &  &  &  & \Circle{} rotations  &  & \\
  &  &  &  & \ding{56} permutations  &  & \\
\midrule
\multirow{3}{3cm}{Overlap Matrix~\cite{sadeghi2013metrics}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{REMatch~\cite{de2016comparing}} & \multirow{3}{3cm}{\circled{C} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} & 
\CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \CheckmarkBold{} permutations  &  & \\
\midrule
\multirow{3}{3cm}{sGDML~\cite{Chmiela2018}} & \multirow{3}{3cm}{\circled{A}  1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\CheckmarkBold{}} &  \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
  &  &  &  & \CheckmarkBold{} rotations  &  & \\
  &  &  &  & \Circle{} permutations\footnote{Only invariant to the group of permutations represented in the training data}  &  & \\
\bottomrule
\end{longtable}
\end{tiny}



% \pagebreak
% \begin{tiny}
% \begin{longtable}{llcclcc}
% \caption{Atomistic systems can be represented in a myriad of ways. Some descriptions are designed to emphasise particular aspects of a system, while others aim to disambiguate similar chemical or physical principles across a wide range of molecules or materials. The set of desirable properties in a representation thus depends on the task at hand. The following overview gives a coarse characterization of the most popular representations.
% We distinguish between four computational efficiency classes \circled{A} - \circled{D} in descending order, depending on the number of considered many-body terms in the descriptor. The efficiency class additionally reflects if a representation relies on particularly expensive operations (e.g. a hierarchical processing or matching of inputs).
% Furthermore, we indicate if a representation is unique and able to encode any physical state of the system unambiguously. Note, that this property may not be crucial in practice, because ML models only have to generalize across a relatively narrow scope of inputs.
% The symbols \CheckmarkBold{} and \ding{56} show if a descriptor satisfies a certain property or not, while \Circle{} means that a property is partly satisfied.}\\
% \toprule
%  & & \multirow{1}{3cm}{\textbf{Comp. efficiency}} & \textbf{Periodic}  & \textbf{Uniq.}  & \textbf{Invariances} & \textbf{Global} & \textbf{Smooth}\\
% \toprule
% \multicolumn{7}{l}{} \\
% \endhead
% \multicolumn{7}{l}{\textbf{Descriptors}} \\
% \toprule
% \multirow{3}{3cm}{Atom-centered Symmetry Functions (ASCF)~\cite{behler2011atom}}  & \multirow{3}{*}{\circled{B} 1,2,3-body terms, cut-off} & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Smooth Overlap of Atomic Positions (SOAP)~\cite{0444_Bartok2013}} & \multirow{3}{3cm}{\circled{B} density based, $\text{SO}_3$ integration} & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}   & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Coulomb Matrix (CM)~\cite{rupp2012fast}} & \multirow{3}{*}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\CheckmarkBold{}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \ding{56} permutations  &  & \\
% \hline
% \multirow{3}{3cm}{Sine Matrix~\cite{faber2015crystal}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \ding{56} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Ewald Sum Matrix~\cite{faber2015crystal}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \ding{56} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Bag of Bonds (BoB)~\cite{0161_Hansen2015}}  & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\ding{56}} & \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \Circle{} permutations\footnote{Partial permutation invariance via feature sorting}  &  & \\
% \hline 
% \multirow{3}{3cm}{Faber-Christensen-Huang-Lilienfeld (FCHL)~\cite{christensen2020fchl}} & \multirow{3}{3cm}{\circled{C} 1,2,3-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Spectrum of London and Axilrod-Teller-Muto potential (SLATM)~\cite{faber2018alchemical}} & \multirow{3}{3cm}{\circled{D} 1,2,3,4-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline
% \multirow{3}{3cm}{Many-body Tensor Representation (MBTR)~\cite{huo2017unified}} & \multirow{3}{3cm}{\circled{C} 1,2,3-body terms} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} &
% \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline
% \multirow{3}{3cm}{Atomic cluster expansion~\cite{drautz2019atomic}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms}  & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\

% \hline 

% \multicolumn{7}{l}{} \\
% \multicolumn{7}{l}{\textbf{NN architectures}} \\
% \toprule
% \multirow{3}{3cm}{Deep Potential - Smooth Edition (DeepPot-SE)~\cite{zhang2018deep,zhang2018end}} & \multirow{3}{3cm}{\circled{B} 1,2,3-body terms, cut-off} & \multirow{3}{*}{\CheckmarkBold{}}  & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{MPNN/SchNet~\cite{0336_schutt2017quantum,0338_schutt2018schnet}} & \multirow{3}{3cm}{\circled{B} 1,2-body terms, hierarchical} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Cormorant~\cite{anderson2019cormorant}} & \multirow{3}{3cm}{\circled{B} 1,2-body terms, hierarchical} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\CheckmarkBold{}} & \CheckmarkBold{} translations  &  \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Tensor Field Networks~\cite{thomas2018tensor}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\ding{56}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
%  \hline

% \multicolumn{7}{l}{} \\
% \multicolumn{7}{l}{\textbf{Similarity metrics}} \\
% \toprule

% \multirow{3}{3cm}{Root mean square deviation of atomic positions (RMSD)~\cite{sadeghi2013metrics}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}  & \multirow{3}{*}{\ding{56}} 
% & \Circle{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
%   &  &  &  & \Circle{} rotations  &  & \\
%   &  &  &  & \ding{56} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{Overlap Matrix~\cite{sadeghi2013metrics}} & \multirow{3}{3cm}{\circled{A} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{REMatch~\cite{de2016comparing}} & \multirow{3}{3cm}{\circled{C} 1,2-body terms, input matching} & \multirow{3}{*}{\ding{56}}   & \multirow{3}{*}{\ding{56}} & 
% \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\ding{56}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \CheckmarkBold{} permutations  &  & \\
% \hline 
% \multirow{3}{3cm}{sGDML~\cite{Chmiela2018}} & \multirow{3}{3cm}{\circled{A}  1,2-body terms} & \multirow{3}{*}{\CheckmarkBold{}}   & \multirow{3}{*}{\CheckmarkBold{}} &  \CheckmarkBold{} translations  & \multirow{3}{*}{\CheckmarkBold{}} & \multirow{3}{*}{\CheckmarkBold{}}\\
%   &  &  &  & \CheckmarkBold{} rotations  &  & \\
%   &  &  &  & \Circle{} permutations\footnote{Only invariant to the group of permutations represented in the training data}  &  & \\
% \hline 
% \label{tab:descriptors}
% \end{longtable}
% \end{tiny}

